How Peer Effects Influence Energy Consumption

This paper analyzes the impact of peer effects on electricity consumption of a network of rational, utility-maximizing users. Users derive utility from consuming electricity as well as consuming less energy than their neighbors. However, a disutility is incurred for consuming more than their neighbors. To maximize the profit of the load-serving entity that provides electricity to such users, we develop a two-stage game-theoretic model, where the entity sets the prices in the first stage. In the second stage, consumers decide on their demand in response to the observed price set in the first stage so as to maximize their utility. To this end, we derive theoretical statements under which such peer effects reduce aggregate user consumption. Further, we obtain expressions for the resulting electricity consumption and profit of the load serving entity for the case of perfect price discrimination and a single price under complete information, and approximations under incomplete information. Simulations suggest that exposing only a selected subset of all users to peer effects maximizes the entity's profit.

==> Sections/Introduction_Short.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is Introduction.tex (part of Peer_Effects.tex)
% author: Datong Zhou
% last edited: Oct 26, 2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% !TEX root = ../Peer_Effects.tex

\section{Introduction}
\label{sec:Introduction}
Energy efficiency programs have emerged as a viable resource to yield economic benefits to utility systems and to reduce the amount of greenhouse gas emissions. Demand-side management aims to modify consumer demand through financial incentive schemes and to induce behavioral changes through education. Specifically, users are offered rewards to conserve energy during peak hours or to shift usage to off-peak times. With communications and information technology constantly improving, which are characteristic elements of today's smart grid, demand-side management technologies are becoming increasingly feasible.

Previous academic work by psychologists, political scientists, and behavioral economists has found that social comparisons can have a significant impact on people's behavior, exploiting the willingness of individuals to conform to a standard, receive social acclaim, or simply the belief that other people's choices are informative in the presence of limited or imperfect information \cite{Akerlof:2000aa, Mani:2013aa}. 

Motivated by this line of academic work and the pressing need to improve energy efficiency, various companies and groups, for instance \texttt{OPOWER}, have conducted randomized control trials to investigate the impact of peer effects on energy consumption of residential households by sending out quarterly energy reports (so called \textit{Home Energy Reports}) to users with a comparison of their usage to their closest neighbors \cite{Ayres:2009aa}. While all experiments unanimously found an average reduction among the highest consuming users of around 1-2$\%$ \cite{Allcott:2011aa}, ambiguous results were found among low consumers, with one study reporting a ``boomerang effect'', that is, an increase of energy demand among the most efficient households.

Network effects in social networks and platforms often exhibit positive externalities, capturing the intuitive fact that an increased amount of platform activity promotes a local increase in platform activity. From a game-theoretic perspective, it is known that an analysis of games under such strategic complements admits well-behaved solutions if utility functions are supermodular with parameters drawn from a lattice \cite{Topkis:1998aa, Zhou:1994aa}. Examples for such games can be found in modeling technology adoption, human capital decisions, and criminal and social networks \cite{Calvo-Armengol:2005aa}. The opposite effect, that is, in games of strategic substitutes where an increased amount of activity leads to local reductions of activity, is observed in information sharing and the provision of public goods \cite{Bramoulle:2007aa}. However, since utility functions in this setting tend to lose the feature of supermodularity, finding equilibria is an inherently hard problem \cite{Jackson:2014aa}, and so these settings have been significantly less studied.

In an attempt to characterize the most influential players in a network, \cite{Ballester:2006aa} develops a quadratic model with continuous action spaces, a parameterization which we employ in this paper. Other research directions aiming at understanding the impact of network effects on social phenomena include diffusion models for the spread of information with the goal of influence maximization \cite{Kempe:2003aa}, repeated games to learn user interactions over time \cite{Acemoglu:2011aa}, or the analysis of systemic risk and stability \cite{Acemoglu:2015aa} in financial networks. The problem of profit maximization of a monopolist selling a divisible good, which is closely related with our work, has been investigated in \cite{Candogan:2012aa}, where the authors assume a constant marginal cost of production. However, to the best of our knowledge, a modeling approach for the impact of peer effects on energy consumption, whose generation typically has quadratic marginal cost, has yet to be formulated. 

In this paper, we propose a two-stage game-theoretic model for the energy consumption of a network of users, serviced by the load-serving entity that is obligated to cover the households' energy demand at all times. We analytically solve for the equilibria of this game under full information of the network structure and users' parameters to characterize the influence of peer effects on aggregate consumption and utility profit, for both the case of perfect price discrimination and a single price valid for all users. For the case of incomplete information, we obtain approximations of the utility's profit, user consumptions, and the optimal pricing scheme. Further, we analyze the profit-maximization problem by selecting the best subset of users to be exposed to peer effects, and present a heuristic solution to this NP-hard selection problem. Lastly, we provide theoretical statements on the properties of users which ensure that the consumption under peer effects is reduced.

The remainder of this paper is organized as follows: Section \ref{sec:Game_Theoretical_Model} presents the two-stage game-theoretic model between the utility and the network of consumers and derives consumption and price equilibria. Based on this model, Section \ref{sec:Theoretical_Statements} presents various theorems on the reduction of consumption in response to the peer effect as well as on the effect of uncertainty of the network structure on the optimal profit. Section \ref{sec:comparison_pricing_schemes} compares the utility's profit under the pricing schemes derived in Section \ref{sec:Game_Theoretical_Model}. Next, the challenge of maximizing the utility's profit by imposing a binary constraint on the number of users exposed to peer effects is formulated and solved with a heuristic approach in Section \ref{sec:profit_max_fixed_price}. Section \ref{sec:Conclusion} concludes. Proofs are relegated to the Appendix. Due to space constraints, some proofs are omitted, but can be found in the full version of this paper \cite{Zhou:aa}.

==> Sections/Minimization_Consumption.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is Minimization_Consumption.tex (part of Peer_Effects.tex)
% author: Datong Zhou
% last edited: Feb 21, 2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% !TEX root = ../Peer_Effects.tex

\section{Minimization of User Consumption}
\label{sec:Minimization_Consumption}
The goal of the pilot programs run by \texttt{OPOWER} was to elicit a reduction in consumer demand with the help of the peer effect. In this section, we assume a fixed uniform price $p$ among all users, which is set by the utility to maximize its profit under normal operation, i.e. in the absence of all peer effects. We investigate the case where the utility can only target a subset of customers, namely $0 \leq m \leq |\mathcal{I}|$, in order to maximize the average treatment effect among the treated (ATT). This situation could arise if the electric utility only has limited resources to treat its customers, or if the state regulation for energy conservation relative to baseline can be satisfied by treating only a fraction of its customer base. The problem is formulated as the following NP-hard Mixed Integer Quadratically Constrained Program (MIQCP):
\begin{equation}\label{eq:targeting_objective_function}
\begin{aligned}
& \underset{\delta_1, \ldots, \delta_n}{\text{minimize}}
& & \sum_{i=1}^n x_i \\
& \text{subject to}
& & \sum_{i=1}^n \delta_i = m,\quad \delta_i\in\lbrace 0, 1\rbrace \\
& & & \mathbf{x} = \left(\Lambda + 2\Delta \Gamma - \Delta \Gamma W\right)^{-1}(\mathbf{a}-p\mathbf{1})
\end{aligned}
\end{equation}
where $\Delta = \text{diag}(\delta_1, \ldots, \delta_n)$. Due to its NP-hardness, \eqref{eq:targeting_objective_function} does not admit a closed form solution, and an analytical solution requires exhaustive search, which is computationally infeasible for any real network of users. Therefore, we make use of a heuristic, which simply computes the consumptions without any network effect, denoted by $\mathbf{\tilde{x}}$, i.e. 
\begin{equation*}
\mathbf{\tilde{x}} = \Lambda^{-1} (\mathbf{a} - p\mathbf{1})
\end{equation*}
and target only the $m$ consumers with the highest consumption, i.e. $\Delta_h = \text{diag}(\delta_{h,1}, \ldots, \delta_{h,n})$, where $\delta_{h,i}=1$ if consumer $i$ is in the set of the $m$ highest consumers, and $0$ otherwise. Lastly, we compare the performance of the heuristic to the case of random selection of households.


==> Sections/Simulations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is Simulations.tex (part of Peer_Effects.tex)
% author: Datong Zhou
% last edited: Oct 26, 2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% !TEX root = ../Peer_Effects.tex

\section{Simulations}
\label{sec:Simulations}
%In this section, we simulate the consumption minimization problem (Section \ref{sec:Minimization_Consumption}), the utility profit under different uniform pricing schemes and varying network strengths $\gamma$ (Section \ref{sec:comparison_pricing_schemes}), and the utility's profit maximization problem (Section \ref{sec:profit_max_fixed_price}) on three basic network topologies, displayed in Figure \ref{fig:basic_networks}.

%\subsection{Consumption Minimization}\label{sec:simulation_cons_minimization}
%We juxtapose the analytical solution to \eqref{eq:targeting_objective_function} to the solution calculated by the heuristic, which computes the hypothetical consumptions in the absence of any network effect $\tilde{\mathbf{x}}$ to target the highest consumers, and a random selection of targeted households. To capture the inherent heterogeneity of consumer behavior, we run a Monte Carlo simulation with $h=2500$ iterations. At each iteration, the parameters $a_i$ and $b_i,~i\in\mathcal{I}$ are drawn from the uniform distributions $a\sim\text{unif}[8,12]$ and $b\sim\text{unif}[0.75, 1.25]$, respectively. Further, let $c_i = 2,~\gamma_i = 0.05~\forall~i\in\mathcal{I}$ be constant during the simulation. With these parameters, the uniform price \eqref{eq:unif_price_complete} evaluates to $p^\ast = 7.5$. Define the cumulative regret $R_m$ of the heuristic for a given number of targeted households $0\leq m \leq n$ as follows:
%\begin{equation}\label{eq:regret_heuristic_cons_minimization}
%R_m = \frac{J_h-J^\ast}{\tilde{J}-J^\ast}\cdot 100\%,
%\end{equation}
%where $J_h, \tilde{J}, J^\ast$ denote the objective for the heuristic, the random selection, and the analytical solution to \eqref{eq:targeting_objective_function}, respectively.
%
%Figure \ref{fig:Minimization_Consumption_Fixed_price} shows the optimal analytical objective $J^\ast$ and the objective under random selection $\tilde{J}$ (dashed line). Further, it displays the percentage of cases in which the heuristic targets the same set of consumers as the analytical solution, and the regret of the heuristic \eqref{eq:regret_heuristic_cons_minimization} for all three network topologies.
%
%It can be seen that the optimal objective is decreasing in the number of users targeted, while the regret peaks for small $m$, but never exceeds $2.5\%$. Compared to random treatment assignment, the optimal solution achieves a reduction of $\approx 2\%$ for $4 \leq m \leq 8$ while the peak demand reduces by $\approx 10\%$. The fact that the regret never exceeds $2.5\%$ indicates that the presented heuristic achieves a good approximation of the optimal solution, which is NP-hard and computationally intractable for larger, real-world networks.

%\begin{figure*}[hbtp]
%{\includegraphics[width=1.0\textwidth]{Figures/Minimization_Consumption.pdf}} \hfill \vspace*{-0.3cm}
%\caption{Average sum of consumptions, percentage of optimal choice of heuristic, and regret for consumption minimization problem under uniform price. 5,000 iterations, $a~\sim~\text{unif}[8,12], b~\sim~\text{unif}[0.75, 1.25], \gamma_i = 0.05~\forall~i$.}
%\label{fig:Minimization_Consumption_Fixed_price}
%\vspace*{-0.01cm}
%\end{figure*}

%\subsection{Utility Profit under Uniform Pricing}
%Figure \ref{fig:Utility_Profit_Pricing_Comparison} shows the average profit $\Pi^\ast$ of the utility under the different pricing schemes and varying network strengths $\gamma$. As can be seen from the first subplot, $\Pi^\ast$ decreases as $\gamma$ increases. This is explained by Theorem \ref{thm:targeted_peer_effects}, which states that the sum of all targeted users' consumptions decreases as $\gamma$ increases, under certain proximity conditions on $\lbrace{a_i\rbrace}_{i=1}^n$ and $\lbrace{b_i\rbrace}_{i=1}^n$. For the distributions on $a_i$ and $b_i$ employed in this simulation and for the special case of two targeted consumers ``1'' and ``2'', these conditions become
%\begin{align*}
%b_1, b_2 < b_\text{max} < 2b_\text{min} \leq 2b_{\text{min}} + 2\gamma\frac{a_{\text{min}}-p}{a_\text{max}-p}\frac{b_\text{min}}{b_\text{max}+3\gamma/2},
%\end{align*}
%which is satisfied by definition of the distribution $F_b$ and $a_{\text{min}} > p$ (Assumption \ref{as:a_strictly_greater_than_p}).
%
%As expected, the profit for perfect price discrimination exceeds the profit under all uniform pricing scenarios. Among the uniform pricing schemes, complete knowledge about the user parameters $\lbrace{a_i\rbrace}_{i=1}^n$ and $\lbrace{b_i\rbrace}_{i=1}^n$ yields the highest profit. For the incomplete information cases, the difference between the profit $\Pi^\ast$ under the pricing strategy without network and with network increases as a function of $\gamma$. This is explained by the second subplot, which depicts the average prices across all iterations for all $\gamma$. As is evident from \eqref{eq:unif_price_incomplete}, only a lower bound on the profit-maximizing price under complete information \eqref{eq:unif_price_complete} is provided. \eqref{eq:optimal_uniform_price} does not incorporate the network effect $\gamma$ at all, which is why the optimal price \eqref{eq:unif_price_complete} remains constant for all $\gamma$.
%
%The question of why to expose users to the network effect, given that $\Pi^\ast$ is decreasing in $\gamma$, is answered by the reduced average and maximum user consumption, which can reduce the capacity and transmission cost of the utility. For the perfect price discrimination case, the maximum user consumption as well as the average profit differ by $\approx 10\%$ for $\gamma=0$ and $\gamma=0.3$, whereas a $\approx 1.5\%$ reduction in utility profit is accompanied by a $\approx 30\%$ reduction of the infinity norm.

%\begin{figure*}[hbtp]
%{\includegraphics[width=1.0\textwidth]{Figures/Full_Targeting_Comparison.pdf}} \hfill \vspace*{-0.3cm}
%\caption{Utility profit, average user consumption, and average maximal user consumption under different uniform prices. Green: Perfect price discrimination \eqref{eq:optimal_price_under_ppd}; Blue: Uniform price under complete information \eqref{eq:unif_price_complete}; Red: Uniform price under incomplete information in the presence of peer effects \eqref{eq:unif_price_incomplete}; Black: Uniform price under incomplete information in the absence of peer effects \eqref{eq:optimal_uniform_price}. 10,000 iterations, $a~\sim~\text{unif}[8,12], b~\sim~\text{unif}[0.75, 1.25]$.}
%\label{fig:Utility_Profit_Pricing_Comparison}
%\vspace*{-0.04cm}
%\end{figure*}

%\subsection{Profit Maximization under Uniform Pricing}
%The same distributions $F_a, F_b$ and parameters $c=2, n=10$ as used in Section \ref{sec:simulation_cons_minimization} are employed for the profit maximization problem of the utility under the uniform price under incomplete information and in the absence of peer effects \eqref{eq:unif_price_complete}. The analytical solution to \eqref{eq:utility_targeting_optimization_problem} is compared to the heuristic which targets users that deviate most from their expected optimal consumption $\mathbb{E}[x_i]$ \eqref{eq:optimal_expected_consumption_unif_price}. The cumulative regret $R_m$ is defined as in \eqref{eq:regret_heuristic_cons_minimization}. Figure \ref{fig:Maximization_Utility_Profit_Fixed_price} shows the average objective for the heuristic, the random selection (dashed line), the percentage of optimal choices under the heuristic, the regret, and the average infinity norm of household consumption.
%
%\begin{figure*}[hbtp]
%{\includegraphics[width=1.0\textwidth]{Figures/Profit_Maximization_FixedPrice.pdf}} \hfill \vspace*{-0.2cm}
%\caption{Average profit, percentage of optimal choice of heuristic, regret, and average infinity norm of consumption for the utility's profit maximization problem under the uniform price \eqref{eq:unif_price_complete}. 2500 iterations, $a~\sim~\text{unif}[8,12], b~\sim~\text{unif}[0.75, 1.25]$.}
%\label{fig:Maximization_Utility_Profit_Fixed_price}
%\vspace*{-0.4cm}
%\end{figure*}
%
%It can be seen that the optimal solution to \eqref{eq:targeting_objective_function} can achieve an increase in profit by $\approx 1\%$ while at the same time reducing the peak consumption by $\approx 4\%$. The heuristic achieves a regret that increases in the number of consumers targeted and peaks at $~25\%$, $~18\%$, and $~10\%$ for the ring, star, and fully connected network, respectively. 


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


